Chromatic PAC-Bayes Bounds for Non-IID Data: Applications to Ranking and Stationary $\beta$-Mixing Processes

Pac-Bayes bounds are among the most accurate generalization bounds for classifiers learned from independently and identically distributed (IID) data, and it is particularly so for margin classifiers: there have been recent contributions showing how practical these bounds can be either to perform model selection (Ambroladze et al., 2007) or even to directly guide the learning of linear classifiers (Germain et al., 2009). However, there are many practical situations where the training data show some dependencies and where the traditional IID assumption does not hold. Stating generalization bounds for such frameworks is therefore of the utmost interest, both from theoretical and practical standpoints. In this work, we propose the first - to the best of our knowledge - Pac-Bayes generalization bounds for classifiers trained on data exhibiting interdependencies. The approach undertaken to establish our results is based on the decomposition of a so-called dependency graph that encodes the dependencies within the data, in sets of independent data, thanks to graph fractional covers. Our bounds are very general, since being able to find an upper bound on the fractional chromatic number of the dependency graph is sufficient to get new Pac-Bayes bounds for specific settings. We show how our results can be used to derive bounds for ranking statistics (such as Auc) and classifiers trained on data distributed according to a stationary {\ss}-mixing process. In the way, we show how our approach seemlessly allows us to deal with U-processes. As a side note, we also provide a Pac-Bayes generalization bound for classifiers learned on data from stationary $\varphi$-mixing distributions.

==> simulations.tex <==
\section{Numerical Simulations}
\label{sec:simulations}

In this section, we compare  the behaviour of the Chromatic \pac-Bayes
Bound,  related to  theorem \ref{th:pbauc},  with regard  to  the test
error  rate. This  comparison  is  made on  six  datasets, namely  the
\emph{image},    \emph{flar solar},   \emph{german},   \emph{titanic},
\emph{splice}  and   \emph{ringnorm}  datasets,  provided   by  Gunnar
R\"{a}tsch\footnote{\url{http://ida.first.fraunhofer.de/projects/bench}}.
For each  dataset, $100$ random  realizations of training  and testing
sets  are  available.  We  have   chosen  $20$  of  them  to  run  the
experiments.

\marie{J'ai zapp\'e \emph{twonorm} car les r\'esultats en classif sont
  \'etranges (quasiment pas d'erreur, et biais = false, \'evidemment).
  \`A voir plus tard\dots}

We have  paired positive with  negative observations, as  described in
Section \ref{sec:example_ranking}. For all  datasets, we have used the
training and testing  partitions as they were defined,  except for the
testing sets  whose size  was greater than  $500$. For the  latter, we
have picked out $500$ observations so that the size $\ell^{+}\ell^{-}$
of  the actual test  set is  limited. The  different sample  sizes are
reported  in table  \ref{tab:sample_size}. \marie{Justifier  les $500$
  exemples en test, autrement que  ``parce qu'on a un serveur en rade,
  et qu'on est limite en temps''.}


\begin{table*}[htb]
  \centering

  \caption{Elements concerning the size of the  datasets.} 
  
  \vspace{0.35cm}
  
  \begin{tabular}{>{\centering}p{1.9cm} || 
      >{\centering}p{1.9cm} | >{\centering}p{1.9cm} | >{\centering}p{1.9cm} || 
      >{\centering}p{1.9cm} | >{\centering}p{1.9cm} | >{\centering}p{1.7cm} c@{\hspace{0cm}} }
    \hline
    Dataset & \#Training  & \#Pos.\,/\,Neg. & Pos.$\times$Neg. & \#Testing &
    \#Pos.\,/\,Neg.  & Pos.$\times$Neg. & \\ 
    \hline
    Image & 1300 &  & & 500 & & & \\
    Flare solar & 666 & 367 / 300 & 109723 & 400 & 223  / 178
    &  39450 & \\
    German & 700 & 211 / 489 & 103072 & 300 & 89 / 211 & 18772
    & \\
    Titanic & 150 & 50 / 101  & 4952 & 500 & 159 / 341 & 54044
    & \\
    Splice & 1000 & 483 / 517 & 249509 & 500 & 243 / 257 &
    62338  & \\
    Twonorm & 400 & 200 / 200 & 39919 & 500 & 248 / 252 & 62436 & \\
    \hline
  \end{tabular}

  \flushleft{\small Number of observations in the original training and the
    testing sets. For the 20 realizations, the average number of the
    positive and negative observations, and the average size of the
    bipartite ranking problems are also reported.} 

  \label{tab:sample_size}
\end{table*}

We have  run a SVM  cutting plane algorithm  \cite{Sonnenburg:scpa} on
each training  set, and  have computed the  average error rate  on the
corresponding testing  set. The  Chromatic \pac-Bayes Bound  error has
been  estimated  on  the  training  set, according  to  the  following
expression:
%
\begin{equation*}
  e_Q = \hat{e}_Q + \frac{1}{\underline{\ell}} 
  \sqrt{
    \frac{
      \frac{\mu^2}{2} + \ln \frac{\underline{\ell} + 1}
      {\delta}}
    {2}} \, ,
\end{equation*}
%
where $\mu^2  = \bfw^{\text{T}}\bfw$ is  related to the margin  of the
classifier.    \marie{R\'ef\'erencer   la    fin    de   la    section
  \ref{sec:example_ranking} o\`u alors  tu ne vas pas en  dire plus ?}
For each  dataset, the average  variation of both errors  according to
the    soft-margin   parameter   $C$,    is   displayed    in   figure
\ref{fig:results}. 

\begin{figure*}
  \centering
  \caption{Average variation of the Chromatic \pac-Bayes bounded error
    and the test error rate.}

  \vspace{0.35cm}

  \begin{tabular}{c c c}
    \emph{image} & \emph{flare solar} &  \emph{german} \\
    & 
    \includegraphics[scale=0.3]{results/flare-solar} & 
    \includegraphics[scale=0.3]{results/german} \\
    \emph{titanic} & \emph{splice}  & \emph{ringnorm} \\
    \includegraphics[scale=0.3]{results/titanic} & 
    \includegraphics[scale=0.3]{results/splice} & 
    \includegraphics[scale=0.3]{results/ringnorm} \\
  \end{tabular}
  \label{fig:results}
  \flushleft{\small{On the abscissa, different values of $C$. The
      dashed blue line  represents the average  error rate,  while the
      cyan line is the average Chromatic \pac-Bayes bounded error
      rate. The square on each curve points the smallest value.}} 
\end{figure*}

One can note that\dots

\marie{Discuter  sur  ce qu'on  va  dire  de  ces courbes  +  quelques
  commentaires  sur le  fait  que  ça sera  vachement  mieux avec  des
  priors. Sinon $\delta=1\%$ sur ces  courbes, mais de toute facon, on
  va  recalculer les  erreurs avec  la super  descente de  gradient de
  Liva ? }

